Offline Reinforcement Learning for LLM Multi-Step Reasoning

Improving the multi-step reasoning ability of large language models (LLMs) with offline reinforcement learning (RL) is essential for quickly adapting them to complex tasks. While Direct Preference Optimization (DPO) has shown promise in aligning LLMs with human preferences, it is less suitable for multi-step reasoning tasks because (1) DPO relies on paired preference data, which is not readily available for multi-step reasoning tasks, and (2) it treats all tokens uniformly, making it ineffective for credit assignment in multi-step reasoning tasks, which often come with sparse reward. In this work, we propose OREO (Offline Reasoning Optimization), an offline RL method for enhancing LLM multi-step reasoning. Building on insights from previous works of maximum entropy reinforcement learning, it jointly learns a policy model and value function by optimizing the soft Bellman Equation. We show in principle that it reduces the need to collect pairwise data and enables better credit assignment. Empirically, OREO surpasses existing offline learning methods on multi-step reasoning benchmarks, including mathematical reasoning tasks (GSM8K, MATH) and embodied agent control (ALFWorld). The approach can be extended to a multi-iteration framework when additional resources are available. Furthermore, the learned value function can be leveraged to guide the tree search for free, which can further boost performance during test time.

==> latex/max_ent_rl.tex <==
\subsection{Maximum-Entropy RL}
\shibo{As mentioned in slack, I temporarily moved this part to appendix, since I believe the current section 3 is concise and self-contained. We can discuss more details}

Maximum-entropy reinforcement learning~\whj{cite} is an extension to standard RL which maximizes the weighted sum of the accumulated reward and the entropy of the policy, namely
\begin{equation}
    J_\text{MaxEnt}(\pi)=\mathbb E_{\tau\sim\pi}\left[\sum_{t\ge 0}r(\mathbf s_t,\mathbf a_t)+\beta\mathcal H(\pi(\cdot\mid\mathbf s_t))\right].
\end{equation}
Since the KL divergence can be written as
\begin{align*}
    &\operatorname{KL}[\pi(\cdot\mid \mathbf s)\|\pi_\text{ref}(\cdot\mid \mathbf s)] \\
    &=\mathbb E_{\mathbf a\sim\pi(\cdot\mid \mathbf s)}[\log\pi(\mathbf a\mid \mathbf s)-\log\pi_\text{ref}(\mathbf a\mid \mathbf s)],
\end{align*}
the RLHF objective can be rewritten as
\begin{align*}
    &J_\text{RLHF}(\pi) \\
    &=\mathbb E_{\tau\sim\pi}\biggl[\sum_{t\ge 0}r(\mathbf s_t,\mathbf a_t) \\
    &\quad -\beta\log\pi(\mathbf a_t\mid\mathbf s_t)+\beta\log\pi_\text{ref}(\mathbf a_t\mid\mathbf s_t)\biggr] \\
    &=\mathbb E_{\tau\sim\pi}\biggl[\sum_{t\ge 0}r(\mathbf s_t,\mathbf a_t)+\beta\log\pi_\text{ref}(\mathbf a_t\mid\mathbf s_t) \\
    &\quad +\beta\mathcal H(\pi(\cdot\mid\mathbf s_t)\biggr],
\end{align*}
\whj{This looks ugly. Any ideas?}
that is, maximum-entropy RL with reward $r(s,a)+\beta\log\pi_\text{ref}(a\mid s)$.

The soft Q-function is defined by~\whj{cite}
\begin{equation}
\small
\begin{split}
    &Q(\mathbf s_t,\mathbf a_t)=r(\mathbf s_t,\mathbf a_t)+ \\
    &\mathbb E_{(\mathbf s_{t+1},\ldots)\sim\pi}\left[\sum_{l\ge 1}r(\mathbf s_{t+l},\mathbf a_{t+l})+\beta\mathcal H(\pi(\cdot\mid\mathbf s_{t+l}))\right],
\end{split}
\end{equation}
and the soft value function is defined by
\begin{equation}
    V(\mathbf s_t)=\log\sum_{\mathbf a}\exp Q(\mathbf s_t,\mathbf a).
\end{equation}
It can be proved that~\whj{cite} the optimal policy satifies
\begin{equation}
    \pi(\mathbf a_t\mid\mathbf s_t)=\exp\left(\frac 1\beta(Q^*\mathbf(\mathbf s_t,\mathbf a_t)-V^*(\mathbf s_t)\right),
\end{equation}
where $Q^*$ and $V^*$ denote the optimal soft Q-function and optimal value function. There is a soft version of the Bellman equation~\whj{cite}
\begin{equation}
    Q(\mathbf s_t,\mathbf a_t)=r(\mathbf s_t,\mathbf a_t)+\mathbb E_{\mathbf s_{t+1}}[V(\mathbf s_{t+1})].
\end{equation}
